Non-Line-of-Sight Tracking and Mapping with an Active Corner Camera

The ability to form non-line-of-sight (NLOS) images of changing scenes could be transformative in a variety of fields, including search and rescue, autonomous vehicle navigation, and reconnaissance. Most existing active NLOS methods illuminate the hidden scene using a pulsed laser directed at a relay surface and collect time-resolved measurements of returning light. The prevailing approaches include raster scanning of a rectangular grid on a vertical wall opposite the volume of interest to generate a collection of confocal measurements. These are inherently limited by the need for laser scanning. Methods that avoid laser scanning track the moving parts of the hidden scene as one or two point targets. In this work, based on more complete optical response modeling yet still without multiple illumination positions, we demonstrate accurate reconstructions of objects in motion and a 'map' of the stationary scenery behind them. The ability to count, localize, and characterize the sizes of hidden objects in motion, combined with mapping of the stationary hidden scene, could greatly improve indoor situational awareness in a variety of applications.

==> NLOS Tracking and Mapping Merge/notation.tex <==
% Begin copied directly from main document source file
\def\xvec{\mathbf{x}}
\def\lvec{\mathbf{p}_{\rm l}} % laser spot
\def\pvec{\mathbf{p}_{\rm s}} % point on hidden surface
\def\cvec{\mathbf{p}_{\rm f}} % point on floor in sensor pixel

% \def\cvecmid{\mathbf{c}_{\rm mid}} % overridden below
% \def\pvecmid{\mathbf{p}_{\rm mid}}
% \def\hiddensurf{\mathcal{S}}
% \def\camerapix{\mathcal{P}}
% \def\bvec{\mathbf{b}}

\def\svec{\mathbf{s}}
\def\sfg{\svec_{\rm fg}}
\def\sbg{\svec_{\rm oc}}
\def\psivecfg{\boldsymbol{\psi}_{\rm fg}}
\def\psivecbg{\boldsymbol{\psi}_{\rm oc}}
\def\thetavec{\boldsymbol{\theta}}
\def\alphafg{a_{\rm fg}}
\def\alphabg{a_{\rm oc}}
\def\rfg{r_{\rm fg}}
\def\rbg{r_{\rm oc}}
\def\pmin{\theta_{\rm min}}
\def\pmax{\theta_{\rm max}}
\def\pmid{\theta_{\rm mid}}
\def\xvec{\mathbf{x}}
\def\ffg{f_{\rm fg}}
\def\gfg{g_{\rm fg}}
\def\fbg{f_{\rm bg}}
\def\gbg{g_{\rm bg}}
\def\smatfg{\mathbf{S}_{\rm fg}}
\def\smatbg{\mathbf{S}_{\rm bg}}
\def\smat{\mathbf{S}}
\def\lnorm{\mathbf{n}_{\lvec}}
\def\cnorm{\mathbf{n}_{\cvec}}
\def\planenorm{\mathbf{n}_{\rm plane}}
\def\pplane{\pvec_{\rm plane}}
\def\pnorm{\mathbf{n}_{\pvec}}
\def\psivecfghat{\widehat{\boldsymbol{\psi}}_{\rm fg}}
\def\psivecbghat{\widehat{\boldsymbol{\psi}}_{\rm bg}}
% End copied directly from main document source file

\def\sfg{\svec_{\rm fg}}
\def\sbg{\svec_{\rm oc}}
\def\thetavec{\boldsymbol{\theta}}
\def\psivecfg{\boldsymbol{\psi}_{\rm fg}}
\def\psivecbg{\boldsymbol{\psi}_{\rm oc}}

\def\psivecfghat{\widehat{\boldsymbol{\psi}}_{\rm fg}}
\def\psivecbghat{\widehat{\boldsymbol{\psi}}_{\rm bg}}

\def\ffg{f_{\rm fg}}
\def\gfg{g_{\rm fg}}
\def\fbg{f_{\rm bg}}
\def\gbg{g_{\rm bg}}
\def\smatfg{\mathbf{S}_{\rm fg}}
\def\smatbg{\mathbf{S}_{\rm bg}}
\def\ael{a_{\rm e}}
\def\bel{b_{\rm e}}
\def\cel{c_{\rm e}}

\def\pvec{\mathbf{p}_{\rm s}}
\def\cvec{\mathbf{p}_{\rm f}}
\def\albedo{a}
\def\deltaArc{\Delta_{\rm arc}^{i,k}}
%\def\lvec{\vb*{l}}
\def\lvec{\mathbf{p}_{\rm l}}
%\def\cvecmid{\mathbf{p}_{\rm f}^{\rm mid}}
% Replaced by Vivek Jun 25
\def\cvecmid{\bar{\mathbf{p}}_{\rm f}}
%\def\pvecmid{\mathbf{p}_{\rm s}^{\rm mid}}
% Replaced by Vivek Jun 25
\def\pvecmid{\bar{\mathbf{p}}_{\rm s}}
\def\lnorm{\mathbf{n}_{\rm l}}
\def\cnorm{\mathbf{n}_{\rm f}}
\def\pnorm{\mathbf{n}_{\rm s}}

% Added by Vivek, changed to bar Jun 25:
\def\cvecmidi{\bar{\mathbf{p}}_{{\rm f},n}}

\def\mline{m_{\rm line}}
\def\cline{b_{\rm line}}
\def\xvec{\mathbf{x}}
\def\vvec{\mathbf{v}}
\def\yvec{\mathbf{y}}

\def\svec{\mathbf{s}}
\def\qvec{\mathbf{q}}
\def\bvec{\mathbf{b}}
\def\vfg{\vvec_{\rm fg}}
\def\vbg{\vvec_{\rm bg}}

\def\deltaR{\Delta_{\rm R}^{n,k}}
\def\deltaArc{\Delta_{\rm arc}^{n,k}}
% \def\lvec{\vb*{l}}

\def\planenorm{\mathbf{n}_{\rm plane}}
\def\pplane{\mathbf{p}_{\rm plane}}
\def\camerapix{\mathcal{P}}
\def\hiddensurf{\mathcal{S}}
\def\tmin{\theta_{\rm min}}
\def\tmax{\theta_{\rm max}}
\def\tmid{\theta_{\rm mid}}
\def\dmin{d_{\rm min}}
\def\dmax{d_{\rm max}}
\def\dint{d_{\rm int}}
\def\Astart{A_{\rm start}}
\def\Astop{A_{\rm stop}}
\def\Amid{A_{\rm mid}}
\def\Bstart{B_{\rm start}}
\def\Bstop{B_{\rm stop}}
\def\Bmid{B_{\rm mid}}
\def\alphafg{\albedo_{\rm fg}}
\def\alphabg{\albedo_{\rm oc}}
\def\rfg{r_{\rm fg}}
\def\rbg{r_{\rm oc}}
\def\pmin{\theta_{\rm min}}
\def\pmax{\theta_{\rm max}}
\def\pmid{\theta_{\rm mid}}
\def\stheta{\svec_\theta}
\def\muvec{\boldsymbol{\mu}}
\def\sigmavec{\boldsymbol{\Sigma}}
\def\fmexact{\svec_{\rm exact}}
\def\fmapprox{\svec_{\rm fast}}
\newcommand{\sign}[1]{{\rm sign}( #1)}

\def\Aground{A_{\rm ground}}
\def\Bground{B_{\rm ground}}
% \newcommand{\norm}[1]{\left\lVert # \right\rVert}

\def\T{{\top}}
